Prioritized Level Replay

Environments with procedurally generated content serve as important benchmarks for testing systematic generalization in deep reinforcement learning. In this setting, each level is an algorithmically created environment instance with a unique configuration of its factors of variation. Training on a prespecified subset of levels allows for testing generalization to unseen levels. What can be learned from a level depends on the current policy, yet prior work defaults to uniform sampling of training levels independently of the policy. We introduce Prioritized Level Replay (PLR), a general framework for selectively sampling the next training level by prioritizing those with higher estimated learning potential when revisited in the future. We show TD-errors effectively estimate a level's future learning potential and, when used to guide the sampling procedure, induce an emergent curriculum of increasingly difficult levels. By adapting the sampling of training levels, PLR significantly improves sample efficiency and generalization on Procgen Benchmark--matching the previous state-of-the-art in test return--and readily combines with other methods. Combined with the previous leading method, PLR raises the state-of-the-art to over 76% improvement in test return relative to standard RL baselines.

==> core/archive/archived_algos.tex <==
% Old version
\begin{algorithm}[htb]
\begin{algorithmic}
    \Require A set of training levels $\Lambda_{\text{train}}$ of environment $E$, A trajectory sampling mechanism $P_\tau$ given a policy and an environment
    \Require Environment level distribution $\hat{P}_L$
    \Require A training process $\mathbf{train}$ for updating the policy
    \While{training}
        \State sample $l \sim{} P_L(l \in \mathcal{L}_E)$
        \State sample $\tau \sim{} P_\tau(\tau | E, \pi, l)$
        \State potentially update policy $\pi \gets \mathbf{train}(\pi, \tau)$ \ed{Fix this line to separate sending experience to training job/experience queue from that of potentially pulling/calculating new policy weights}
    \EndWhile
\end{algorithmic}
 \caption{Regular Training: Uniform Level Sampling}
 \label{alg:regular_training}
\end{algorithm}


\begin{algorithm}[htb]
\begin{algorithmic}
    \Require Environment $E$, a buffer $\mathcal{B}$, and the set $\mathcal{L}_E$ of levels from $E$
    \Require A trajectory sampling mechanism $P_\tau$ given a policy and an environment
    \Require An environment level distribution $P_{L}$
    \Require Buffer-conditional Bernoulli distribution $P_{D}$ for deciding where to sample from
    \Require A scoring function $\mathbf{score}$, and a staleness function $\mathbf{stale}$
    \Require A score-based level distribution $P_S$ and an age-based level distribution $P_A$
    \Require A mixture hyperparameter $\rho \in (0, 1)$ over score- and age-based level distributions
    \Require A training process $\mathbf{train}$ for updating the policy
    %
    \State Training step counter $c \gets 0$
    \While{training}
        \State $c \gets c + 1$
        \State sample decision $d \sim{} P_{D}(d\in{} \{0, 1\} | \mathcal{L}_E, \mathcal{B})$
        \State
        \State // either sample a (potentially new) level from $P_L$ or sample one from the buffer
        \If{$d = 1$}
            \State sample $l \sim{} P_{L}(l \in \mathcal{L}_E)$
        \Else
            \State aggregate scores $S \gets \{(l_i, s_i) | (l_i, s_i, c_i) \in \mathcal{B}\}$
            \State aggregate ages $A \gets \{(l_i, \mathbf{stale}(c, c_i)) | (l_i, s_i, c_i) \in \mathcal{B}\}$
            \State sample $l \sim{} (1-\rho) \cdot P_S(l \in \mathcal{L}_E | S) + \rho \cdot P_A(l \in \mathcal{L}_E | A)$
        \EndIf
        \State
        \State // gather some experience and score it
        \State sample $\tau \sim{} P_\tau(\tau | E, \pi, l)$
        \State compute score $s \gets \mathbf{score}(\tau, \pi)$
        \State
        \State // if the level was already in the buffer, update the score and age, or add it if it's new
        \If{there is $(l_i, s_i, c_i) \in \mathcal{B}$ such that $l_i = l$}
            \State update tuple $(l_i, s_i, c_i) \in \mathcal{B}$ with $s_i \gets s$ and $c_i \gets c$
        \Else
            \State append new tuple $(l, s, c)$ to $\mathcal{B}$
        \EndIf
        \State 
        \State potentially update policy $\pi \gets \mathbf{train}(\pi, \tau)$ \ed{Fix this line to separate sending experience to training job/experience queue from that of potentially pulling/calculating new policy weights}
    \EndWhile
\end{algorithmic}
\caption{Prioritized Level Replay}
\label{alg:thealgo}
\end{algorithm}




% PG Algorithm with prioritized level replay
\begin{algorithm}[htb]
\begin{algorithmic}
    \Require Training levels $\Lambda_{\text{train}}$ of environment $\mathcal{E}$, policy $\pi_{\theta}$, rollout length $T$, number of epochs $N_{e}$, batch size $N_{b}$, policy update function $\mathcal{U}(\mathcal{B}, \theta) \rightarrow \theta'$.
    \State Initialize level scores $\mathbf{S} = \mathbf{0}$, partial level scores $\Tilde{\mathbf{S}} = \mathbf{0}$, and level staleness values $\mathbf{A} = \mathbf{0}$ 
    \State Initialize experience buffer $\mathcal{B} = \varnothing$
    \State Initialize $N_b$ parallel environment instances, $\mathbf{E}$
    \For{$i=k$ \textbf{to} $N_{b}$}
        \State $\mathbf{E}[k] \sim \text{Uniform}(\Lambda_{\text{train}})$
    \EndFor
    \For{$e=1$ \textbf{to} $N_{e}$}
        \State $\mathcal{B} \leftarrow \varnothing$
        \For{$k=1$ \textbf{to} $N_{b}$}
            \State $\mathcal{B}\;\cup\;\textbf{collect\_experiences}(k, \mathbf{E}, \Lambda_{\text{train}}, \pi_{\theta}, T, \mathbf{S}, \Tilde{\mathbf{S}}, \mathbf{A})$ \algorithmiccomment{Using Algorithm \ref{alg:collect_exp_prioritized_level_replay}}
        \EndFor
        \State $\theta \leftarrow \mathcal{U}(\mathcal{B}, \theta)$
    \EndFor
\end{algorithmic}
\caption{Generic PG algorithm with prioritized level replay}
\label{alg:pg_level_replay}
\end{algorithm}

% Prioritized Level Replay experience collection subroutine
\begin{algorithm}[htb]
\begin{algorithmic}
    \Require Worker index $k$, parallel environments $\mathbf{E}$, training levels $\Lambda_{\text{train}}$, current level $l$,\\policy $\pi_{\theta}$, rollout length $T$, score function $f$, level scores $\mathbf{S}$, partial scores $\Tilde{\mathbf{S}}$, staleness values $\mathbf{A}$
    \Ensure Experience buffer $\mathcal{B}$
    
    \State Initialize $\mathcal{B} = \varnothing$
    \State Set current level $l = \mathbf{E}[k]$ 
    \State Observe current state $s_0$, termination flag $d_0$
    \If{$d_0$}
        \State Choose current level $l \sim \mathcal{P}(\Lambda_{\text{train}}|\mathbf{S},\mathbf{A})$ and  $\mathbf{E}[k] \leftarrow l$
        \State Update staleness values $\mathbf{A}[l] \leftarrow \mathbf{A}[l] + \mathbf{1}$, $\mathbf{A}[l] \leftarrow 0$ 
        \State Observe initial state $s_0$
    \EndIf
    \State Choose $a_0 \sim \pi_{\theta}(\cdot|s_0)$
    \State t = 1
    \State Initialize episodic trajectory buffer $\tau = \varnothing$
    \While{$t < T$}
        \State Observe $(s_t, r_t, d_t)$
        % \State $h \leftarrow (s_{t-1}, a_{t-1}, s_t, r_t, d_t, \log\pi_{\theta}(a))$
        % \State $\mathcal{B}\;\cup \leftarrow (s_{t-1}, a_{t-1}, s_t, r_t, d_t, \log\pi_{\theta}(a))$ 
        % \State $\mathcal{B}\leftarrow \mathcal{B}\;\cup h$
        % \State $\tau\leftarrow \tau \cup h$
        \State $\mathcal{B}\leftarrow \mathcal{B}\;\cup (s_{t-1}, a_{t-1}, s_t, r_t, d_t, \log\pi_{\theta}(a))$
        \State $\tau\leftarrow \tau \cup (s_{t-1}, a_{t-1}, s_t, r_t, d_t, \log\pi_{\theta}(a))$
        \If{$d_t$}
            \State Update level score $\textbf{S}[l] \leftarrow f(\tau, \Tilde{\mathbf{S}}[l])$ and partial score  $\Tilde{\mathbf{S}}[l] \leftarrow 0$
            \State $\tau \leftarrow \varnothing$
            \State Update current level $l \sim \mathcal{P}(\Lambda_{\text{train}}|\mathbf{S},\mathbf{A})$ and $\mathbf{E}[k] \leftarrow l$
            \State Update staleness values $\mathbf{A}[l] \leftarrow \mathbf{A}[l] + \mathbf{1}$, $\mathbf{A}[l] \leftarrow 0$ 
        \EndIf
        \State Choose $a_{t+1} \sim \pi_{\theta}(\cdot|s_t)$
        \State $t \leftarrow t + 1$
    \EndWhile
    \If{not $d_t$}
        \State $\Tilde{\mathbf{S}}[l] \leftarrow (f(\tau), |\tau|)$
    \EndIf
\end{algorithmic}
\caption{Collect experiences with prioritized level replay}
\label{alg:collect_exp_prioritized_level_replay}
\end{algorithm}



% Algorithm 5 from Sep 20
\begin{algorithm}[htb]
\begin{algorithmic}
    \Require Environment $E$, a buffer $\mathcal{B}$, and the set $\mathcal{L}_E$ of levels from $E$
    \Require A global episode counter $c$
    \Require A trajectory sampling mechanism $P_\tau$ given a policy and an environment
    \Require An environment level distribution $P_{L}$
    \Require Buffer-conditional Bernoulli distribution $P_{D}$ for deciding where to sample from
    \Require A scoring function $\mathbf{score}$
    \Require A score-based level distribution $P_S$ and an age-based level distribution $P_A$
    \Require A mixture hyperparameter $\rho \in (0, 1)$ over score- and age-based level distributions
    \Ensure A trajectory $\tau$
    %

        \State globally update $c \gets c + 1$
        \State sample decision $d \sim{} P_{D}(d\in{} \{0, 1\} | \mathcal{L}_E, \mathcal{B})$
        \State
        \State // either sample a (potentially new) level from $P_L$ or sample one from the buffer
        \If{$d = 1$}
            \State sample $l \sim{} P_{L}(l \in \mathcal{L}_E)$
        \Else
            \State sample $l \sim{} (1-\rho) \cdot P_S(l \in \mathcal{L}_E | \mathcal{B}) + \rho \cdot P_A(l \in \mathcal{L}_E | \mathcal{B}, c)$
        \EndIf
        \State
        \State // gather some experience and score it
        \State sample $\tau \sim{} P_\tau(\tau | E, \pi, l)$
        \State compute score $s \gets \mathbf{score}(\tau, \pi)$
        \State
        \State // if the level was already in the buffer, update the score and age, or add it if it's new
        \If{there is $(l_i, s_i, c_i) \in \mathcal{B}$ such that $l_i = l$}
            \State update tuple $(l_i, s_i, c_i) \in \mathcal{B}$ with $s_i \gets s$ and $c_i \gets c$
        \Else
            \State append new tuple $(l, s, c)$ to $\mathcal{B}$
        \EndIf
        \State 
        \State \Return $\tau$

\end{algorithmic}
\caption{Prioritized Level Replay}
\label{alg:thealgo}
\end{algorithm}

==> core/archive/archived_methods.tex <==
\section{\algoname{}}

Our method builds on the observation that at any given point in training, not all levels are equally useful for improving the policy, as for a given policy parameterization, policy updates based on experiences collected over different levels will result in different amounts of performance improvement on both training and test levels. Our approach aims to learn a dynamic prioritization over training seeds in the form of a sampling distribution $\mathcal{P}_n$, such that sampling training seeds $\xi \sim \mathcal{P}_n$ after the $n$-th episode results in higher average returns on unseen levels than the standard baseline of uniformly sampling training levels throughout training.

Drawing inspiration from active learning and prioritized experience replay techniques from offline RL, we develop a computationally efficient approach that updates $\mathcal{P}_n$ online, requiring no additional gradient updates. Our method assigns a score to each training level, and updates these scores online after each policy update. These level scores are normalized into a probability distribution, from which successive training levels are sampled. In order to achieve reliable performance gains, we found it necessary to increase the weight of a level based on how long ago it was sampled, which we term a level's \emph{staleness}. This section describes these scoring, normalization, and staleness management components of our approach, which together constitute \algoname{}.

\subsection{Scoring Levels}
The assignment of a seed score $S(\xi)$ to each training seed $\xi$ serves as the central component of our method. Over the course of training, the seed score $S(\xi)$ is updated each time the agent reaches a terminal state in the level generated from $\xi$. We use $\mathbf{S}$ to refer to the vector whose elements are the training seed scores, in ascending order of the seed values. The seed-sampling distribution assigns weights that are monotonically increasing with the seed scores. Therefore, useful scoring functions should assign higher scores to levels on which the agent is more likely to experience a trajectory useful for improving its current policy. As the seed scores are updated online after each episode, so is the seed-sampling distribution.

We assume the scoring function $S$ takes the following form over a trajectory $\tau$ of $T$ steps on the level generated from seed $\xi$, and a \emph{scoring metric} $q(t,\tau, \boldsymbol{\lambda}) \rightarrow \mathbb{R}$, parameterized by $\boldsymbol{\lambda}$,

\begin{equation}\label{scoring_function_mean}
\begin{aligned}
S(\xi) = \frac{1}{T}\sum_{t=0}^{T}q(t, \tau, \boldsymbol{\lambda}).
\end{aligned}
\end{equation}

Let $g$ be any aggregation function such as the arithmetic average used in Equation \ref{scoring_function_mean}. Generally, we can assume the scoring function can take the form,
$S(\xi) = g(\{q(t, \tau, \boldsymbol{\lambda}) | 0 < t \le T \})$ or more generally, $S(\xi) = f(\tau, \theta, \boldsymbol{\lambda})$. We leave the investigation of alternative and learned aggregation functions $g$ and general scoring functions $f$ to future work. In this paper, we investigate the efficacy of two classes of scoring functions: uncertainty scores and temporal-difference (TD) scores, following the form of Equation \ref{scoring_function_mean}. See Table \ref{table_scoring_metrics} for a list of all scoring metrics investigated in this paper. 

\textbf{Uncertainty scores.} We adapt the selection criteria used in uncertainty-based active learning for use as scoring functions, by applying a specific classifier uncertainty metric, such as entropy or min-margin, to the agent's policy at each time step. The level score is then the average of the uncertainty metric across all steps in the trajectory. 

\textbf{Temporal-difference scores.} This class of scoring functions uses a variation of a TD error as the scoring metric at each time step. In particular, we look at the efficacy of using the standard 1-step TD error, $\delta_t = r_t + \gamma V(s_t) -  V(s_t)$, as well as the signed and unsigned generalized advantage estimate (GAE). The GAE is defined as an exponentially-weighted average of k-step advantage estimators, and can be compactly expressed as the discounted sum of successive TD errors \citep{schulman2015high}:

\begin{equation}\label{gae}
\begin{aligned}
A_t^{GAE(\gamma,\lambda)} = \sum_{k=t}^T(\gamma\lambda)^{t-k}\delta_t.
\end{aligned}
\end{equation}

As our experiments train the agent's policy using PPO with GAE, the absolute value $|A_t^{GAE(\gamma,\lambda)}|$ is equivalent to the L1 value loss. 

\begin{table}[!htbp]
\renewcommand{\arraystretch}{1.6}
\caption{Choices of scoring metrics $q(\xi)$ investigated in this work.}
\label{table_scoring_metrics}
\centering
\begin{tabular}{@{}lllll@{}}
\toprule
\textbf{Scoring metric} & \textbf{$q(t, \tau, \boldsymbol{\lambda})$} \\ \midrule
Policy entropy & $\sum_a{\pi(a, s_t) \log \pi(a, s_t)}$ \\
Policy min-margin & $\max_{a} \pi(a, s_t) - \max_{a \neq \max_{a} \pi(a, s_t)} \pi(a, s_t)$ \\
Policy least-confidence & $1 - \max_{a}\pi(a, s_t)$ \\
Unsigned 1-step TD error & $|\delta_t|$ \\
GAE & $\sum_{k=t}^T(\gamma\lambda)^{t-k}\delta_t$ \\
Unsigned GAE (L1 value loss) & $|\sum_{k=t}^T(\gamma\lambda)^{t-k}\delta_t|$ \\ 
\bottomrule
\end{tabular}
\end{table}

\subsection{Prioritizing Levels}    
The sampling weights over the training seeds are computed by passing the training seed scores $\mathbf{S}$ element-wise  into a monotonically increasing function $h: \mathbb{R} \mapsto \mathbb{R^+}$, which we call the \emph{prioritization function}. The outputs of $h$ over the training seeds are then normalized to sum to $1$, yielding a valid distribution. During normalization, each of the seed priorities, $h(S(\xi))$, is raised to $1/\beta$, where $\beta$ is a temperature parameter. The prioritization function $h$ specifies how relative differences in seed scores translate into differences in assigned probability mass under the level-sampling distribution:

\begin{equation}\label{prioritization}
\begin{aligned}
P(\xi) = \frac{h(S(\xi))^{1/\beta}}{\sum h(S(\xi))^{1/\beta}}.
\end{aligned}
\end{equation}

This paper investigates the efficacy of several prioritization functions, two of which have been proven effective in the setting of prioritized experience replay: The identity function, $h(\xi) = S(\xi)$, which leads to what we call \emph{proportional prioritization}, and the inverse rank function, which leads to what we call \emph{rank prioritization}. We also investigate \emph{greedy prioritization}, in which only the seed with the highest score receives a nonzero weighing. See Table \ref{table_prioritization_functions} for the explicit definitions of all prioritization functions investigated in this paper.

\begin{table}[!htbp]
\renewcommand{\arraystretch}{1.6}
\caption{Choices of prioritization functions investigated in this work.}
\label{table_prioritization_functions}
\centering
\begin{tabular}{@{}lllll@{}}
\toprule
\textbf{Prioritization} & \textbf{$h(\xi)$} \\ \midrule

Proportional & $S(\xi)$ \\
Rank & $1/\text{rank}(S(\xi))$ \\
Greedy & $\delta_{\xi,\max_\xi S(\xi)}$ \\
\bottomrule
\end{tabular}
\end{table}

\subsection{Managing Staleness}

In general, the prioritization function $h$ can lead to repeated concentration of the probability mass of $\mathcal{P}(n)$ on the same few seeds for several policy updates. This leads to the same small set of levels being sampled for every training episode, leading to overfitting. We prevent this degenerate outcome by explicitly mixing the sampling distribution with a \emph{staleness distribution}, which assigns probability mass to each training seed $\xi$ in proportion to the staleness $\alpha(\xi)$, defined as the number of seeds sampled since $\xi$ was last sampled. The level-sampling distribution then becomes

\begin{equation}\label{staleness}
\begin{aligned}
P_n(\xi) = (1-\rho)\frac{h(S(\xi))^{1/\beta}}{\sum h(S(\xi))^{1/\beta}} + \rho\frac{\alpha(\xi)}{\sum \alpha(\xi)},
\end{aligned}
\end{equation}

where $0 \le \rho \le 1$.

==> core/archive/experiments_old.tex <==
\section{Experimental Setting}
\label{sec:experiments}
We evaluate the effectiveness of \algoname{} on several PCG environments with various combinations of scoring functions and prioritization schemes, and compare against the most common direct level sampling baseline of $P_{\text{train}}(l | \Lambda_{\text{train}}) = \mathbf{Uniform}(l; \Lambda_{\text{train}})$. We train and test on all 16 games in the Procgen Benchmark on the easy difficulty setting and select hard exploration environments from the MiniGrid suite. In addition, we demonstrate that our method, when combined with UCB-DrAC \citep{raileanu2021automatic}, sets a new state-of-the-art on Procgen Benchmark. 

We additionally compare against mixreg \citep{wang2020mixreg}, a data augmentation method that was not published when UCB-DrAC was established as the previous state-of-the-art on Procgen Benchmark.

We further compare against the TSCL Window algorithm, which resembles \algoabbrev{} without staleness sampling and an alternative scoring function based on the magnitude of the slope of recent episodic returns over episode count for each level \citep{Matiisen_2020}. For fairness of comparison, we also evaluate a custom TSCL Window variant that, like \algoabbrev{}, mixes the staleness distribution $P_{C}$ weighted by $\rho$ into its sampling distribution.

In line with the standard baseline for these environments, all our experiments use PPO with GAE for training. For Procgen Benchmark we use the same ResBlock architecture as \citet{cobbe2019procgen} and 200 training levels on the easy setting as in the original baselines, while sampling unseen levels for every test run. 
For MiniGrid, we use a 3-layer CNN architecture based on \citet{igl2019generalization}, and provide approximately 1000 levels of each difficulty per environment during training. Detailed descriptions of the environments, architectures, and hyperparameters used in our experiments (as well as how they were set or obtained) can be found in Appendix~\ref{app:environments}. See Table~\ref{table:scoring_metrics} for the full set of scoring functions $\mathbf{score}(\tau, \pi)$ investigated in our experiments. Additionally, we report results of training on the full level distribution of these MiniGrid environments in Appendix \ref{section:training_on_full_dist}.

\begingroup
\setlength{\tabcolsep}{1pt}
\begin{table}[hbtp]
\caption{Scoring functions investigated in this work.}
\vskip 0.1in
\label{table:scoring_metrics}
\begin{center}
\begin{tabularx}{\linewidth}{p{0.42\linewidth}p{0.5\linewidth}} 
\toprule
\renewcommand{\arraystretch}{1.8}
\textbf{Scoring function} & \textbf{$\mathbf{score}(\tau, \pi)$} \\ 
\midrule
Policy entropy & $\frac{1}{T}\sum_{t=0}^{T} \sum_a{\pi(a, s_t) \log \pi(a, s_t)}$ \\[8pt]
Policy min-margin & \pbox{7cm}{$\frac{1}{T}\sum_{t=0}^{T} (\max_{a} \pi(a, s_t$) $-$\\ $\max_{a \neq \max_{a} \pi(a, s_t)} \pi(a, s_t))$} \\[8pt]
Policy least-confidence & $\frac{1}{T}\sum_{t=0}^{T} (1 - \max_{a}\pi(a, s_t))$ \\[8pt]
1-step TD error & $\frac{1}{T}\sum_{t=0}^{T} |\delta_t|$ \\[8pt]
GAE & $\frac{1}{T}\sum_{t=0}^{T} \sum_{k=t}^T(\gamma\lambda)^{t-k}\delta_t$ \\[8pt]
\pbox{4cm}{Unsigned GAE \\ (L1 value loss)}  & $\frac{1}{T}\sum_{t=0}^{T} \left|\sum_{k=t}^T(\gamma\lambda)^{t-k}\delta_t\right|$ \\ 
\bottomrule
\end{tabularx}
\end{center}
\end{table}
\endgroup

==> core/archive/intro2.tex <==
Our open source implementation is available at \mbox{\url{https://github.com/facebookresearch/level-replay}}.

Environments generated using procedural content generation (PCG) have garnered increasing interest in RL research, leading to a recent surge of PCG environments such as MiniGrid~\citep{gym_minigrid}, Obstacle Tower Challenge~\citep{Juliani_2019}, Procgen Benchmark~\citep{cobbe2019procgen}, and the NetHack Learning Environment~\citep{kttler2020nethack}. Unlike singleton environments, such as those in the Arcade Learning Environment benchmark~\citep{Bellemare_2013}, which are exploitable by memorization and deterministic reset strategies~\citep{ecoffet2019goexplore,DBLP:journals/corr/abs-2004-12919}, PCG environments create novel environment instances algorithmically. 

Throughout this work, we refer to each configurations of the environment which yield PCG environment instances using the generic term \emph{level}. 
Every such level exhibits a unique configuration of underlying factors of variation, such as layout, positions of game entities, asset appearances, or even different rules governing environment transitions, making them a promising target for evaluating systematic generalization in RL~\citep{Risi_2020}. For example, in one environment such as Procgen Benchmark's~\cite{cobbe2019procgen} \emph{Coinrun} environment, a level might specify the particular sequence of stage configurations the environment will need to obtain a coin in; while in \emph{BossFight}, each level determines the shapes and colors of the enemy and projectiles, as well as the background image and colormap. Ultimately, levels can be arbitrarily defined as any selected set of options within the factors of variation of the PCG environment, giving a rich and general scope to this concept. 

Furthermore, in this work we assume only that each level can be associated with a level identifier (e.g.~an index, a random number generator seed, etc.) used by the PCG algorithm to generate a specific level, and that such an identifier is sufficient to reset the environment to a setting with that configuration. For example, in the ProcGren Benchmark, the random number generator seed may serve as such an identifier, since it is sufficient to replay a particular version of, say, BossFight's color/shape configuration while not precluding the environment from being being stochastic in other ways (and thus capable of generating novel experience as the agent acts). This allows for a clean notion of train-test split and testing on held-out levels, in line with the best practices from supervised learning. \textbf{[[TODO: We need to say something about how weak this ``simplifying'' assumption is, relative to other assumptions frequently made in other approaches/environment types.]]}

% Success in the PCG setting requires RL agents to overcome fundamental challenges around learning useful behaviors that generalize across ever-changing observations and transition dynamics. 
Due to the variation among algorithmically-generated levels, a random selection of PCG levels can, in principle, correspond to levels of varying difficulty as well as reveal different---perhaps rare---environment dynamics. This diversity among levels implies that different levels hold differing learning potential for an  agent at any point in training, a fact exploited by methods that both learn to generate levels as well as to solve them \citep{DBLP:conf/gecco/WangLCS19,wang2020enhanced}. 
Here, we focus on the less intrusive setting where we do not have control over level generation, but can instead \emph{replay} (that is, revisit) any previously visited level during training to generate entirely new experiences from it.
% In this setting, current methods train agents by indiscriminately sampling from the training level distribution.

We introduce \algoname{}, illustrated in Figure~\ref{fig:algo_fig}, a method for sampling training levels that exploits this difference among levels. Our method induces a level-sampling distribution that prioritizes levels based on the learning potential of replaying each level anew. Throughout agent training, our method updates a heuristic score appraising the agent's learning potential on a level based on temporal-difference (TD) errors collected along the last trajectory sampled from that level. 
Rather than sampling from the default, typically static (e.g.~uniform), training level distribution, our method samples from a distribution derived from a normalization procedure over these level scores. 
\algoname{} does not make any assumption about how the policy is updated, and is therefore compatible with any RL method.
Furthermore, our method does not rely on some external or general method for quantifying difficulty of a level, but instead derives a level score directly from the policy. The only requirements---satisfied in a wide number of settings where a simulator or game is used to collect experience---are as follows: (i) some notion of ``level'' exists, (ii) such levels can be sampled from the environment in an identifiable way, and (iii) given a level identifier, it is possible to set the environment to that level to be able to collect new experiences from it.

%%% Past work and what's missing/how PLR is different %%%
While previous works in off-policy RL devised effective methods to directly reuse \emph{past} experiences for training \citep{schaul2015prioritized, andrychowicz2017hindsight}, \algoname{} uses past experiences to inform the collection of \emph{future} experiences by assessing how much replaying each level anew will benefit learning. Our method can thus be seen as a forward-view variation of prioritized experience replay, and an online counterpart to this off-policy method.

%%% Detailed investigation of scoring and sampling approaches %%%
This paper makes the following core contributions: 
(i) we introduce a computationally efficient algorithm for adaptively prioritizing levels throughout training using a heuristic-based assessment of the learning potential of replaying each level,
(ii) we empirically demonstrate our method leads to significant gains on 11 of 16 Procgen Benchmark environments and two challenging MiniGrid environments, (iii) we demonstrate our method combines with a previous leading method to set a new state-of-the-art on Procgen Benchmark, and (iv) we provide evidence that our method induces an implicit curriculum over training levels in sparse reward settings.
% Our open source implementation is available at \mbox{\url{https://github.com/facebookresearch/level-replay}}.

==> core/archive/results_discussion_old.tex <==
\section{Results and Discussion}
\algoabbrev{} consistently provides significantly better (or at least on-par) results than direct level sampling. In particular,
we find that:
(i) \algoabbrev{} consistently outperforms both direct level sampling in generalization and sample-efficiency across environments, 
(ii) alternative scoring functions lead to inconsistent improvements across environments, (iii) our method can yield significant additive gains combined with other methods, and (iv) \algoabbrev{} induces an implicit curriculum over training levels, which substantially aids training in hard exploration environments.

\subsection{Procgen Benchmark}
\label{ssec:procgen_benchmark}
Our results in Figure~\ref{fig:procgen_summary} show that \algoabbrev{} with rank prioritization, $\beta = 0.1$ and $\rho = 0.1$, leads to the most substantial improvements across games. This setting yields statistically significant ($p=0.05$) improvements in generalization performance over uniform-sampling on 10 out of 16 environments, according to Welch's t-test.
In comparison, \algoabbrev{} with proportional prioritization provides statistically significant gains over uniform sampling on one more game, but with smaller gains on some games. Notably, gains only occur when the replay distribution considers \emph{both} level scores and staleness, highlighting the importance of staleness-based sampling in keeping scores from drifting off-policy. Figure \ref{fig:procgen_summary} additionally summarizes the mean normalized test return and generalization gap--defined as train return minus test return--throughout training across all 16 games, making the relative strengths of each method immediately apparent. We compute normalized returns according to \citet{cobbe2019quantifying}. As larger generalization gaps indicate overfitting to the training set, we see \algoabbrev{} improves not just sample efficiency but also generalization of the learned policies—outperforming all methods in both regards when used alone, and further still when combined with UCB-DrAC. On the hard setting, our method attains a statistically significant 38.6\% improvement over uniform level-sampling, when directly using the best hyperparameters found in the easy setting. 
Figures
\ref{fig:procgen_test_returns_large},
\ref{fig:procgen_gen_gap_large},
\ref{fig:prop_staleness_spectrum}, \ref{fig:procgen-hard-value_l1},
and Table \ref{tab:ucb-drac-plr-hard} in Appendix~\ref{app:additional_experiments} report these  results in additional detail.

\begin{figure*}[t!]
    \centering
    \includegraphics[width=1.0\textwidth]{figures/plots/procgen_main_summary.pdf}
    \caption{Left: Mean episodic test returns (10 runs) of each method. Each colored $\bigstar$ indicates statistically significant ($p=0.05$) gains in final test performance or sample complexity along the curve, relative to uniform sampling for the PLR-based method of the same color. Center: Mean normalized train and test returns averaged across all games. Right: Mean generalization gaps averaged across all games.}
    \label{fig:procgen_summary}
\end{figure*}

The remaining scoring metrics based on TD-error and classifier uncertainty perform inconsistently across games. While certain games such as BigFish seem amenable to improvements in both training sample complexity and generalization under various \algoname{} scoring metrics, other games, such as Ninja, see no improvement or even degraded sample complexity and generalization. See Figure~\ref{fig:alternative-scoring-results} for an example of this inconsistent effect across games. We find the best-performing variant of TSCL Window does not incorporate staleness information ($\rho = 0$) and also leads to inconsistent outcomes across games, notably significantly worsening performance on StarPilot, as seen in Figure \ref{fig:procgen_summary}.

\begin{figure}[t!]
    \centering
    \includegraphics[width=1.0\linewidth]{figures/plots/bigfish_ninja_compare.pdf}
    % \includegraphics[width=0.5\linewidth]{figures/plots/bigfish_ninja_alt_scoring.pdf}
    \vspace{-.2cm}
    \caption{Two example Procgen Benchmark environments, between which all scoring functions except for L1 value loss show inconsistent improvements to generalization and sample efficiency, with rank prioritization  \mbox{$\beta=0.1$}, and $\rho=0.3$. This inconsistency holds across settings in our grid search.}
    \label{fig:alternative-scoring-results}
\end{figure}

As noted, \algoabbrev{} easily combines with many other methods, as it only modifies the sampling process for the next training level. To demonstrate this fact, we combine our method with UCB-DrAC. Our combined setup trains agents using UCB-DrAC while sampling training levels at the start of each episode using \algoabbrev{}. As summarized in Figure \ref{fig:procgen_summary} and Table \ref{tab:ucb-drac-plr-sota}, UCB-DrAC combined with our method sets a new state-of-the-art on the Procgen Benchmark. The full details of this experiment are provided in Appendix \ref{app:ucb-drac-plr}. 

% TABLE STARTS HERE
\begin{table*}[!htb]

\newcommand\mc[1]{\multicolumn{1}{l}{#1}}

\setlength{\tabcolsep}{2.5pt}
\caption{Comparison of test performance of policies trained on each method. Here PLR makes use of rank prioritization, $\beta=0.1$, and $\rho=0.1$. Following \citet{raileanu2021automatic}, the reported mean and standard deviation per environment is computed by evaluating the final policy's average return on 100 test episodes, aggregated across multiple training runs (10 runs for Procgen Benchmark and 3 for MiniGrid). Each run is initialized with a different training seed. Normalized test returns per run are computed by dividing the average test return per run for each environment by the corresponding average test return of the uniform-sampling baseline over all runs. We then report the means and standard deviations of normalized test returns aggregated across runs. Note, we report the normalized return statistics for Procgen and MiniGrid environments separately.}
\label{tab:ucb-drac-plr-sota}

\begin{center}
\begin{subtable}{\linewidth}
% \centering
\begin{tabular}{l|r r r r| r r}
\toprule
Environment &Uniform &TSCL &mixreg &UCB-DrAC &PLR &UCB-DrAC + PLR\\
\midrule
bigfish&$3.7\pm1.2$&$4.3\pm1.3$&$6.9\pm1.6 $&$8.7\pm1.1 $&$10.9\pm2.8 $&$\mathbf{14.3\pm2.1 }$\\
bossfight&$7.7\pm0.4$&$7.4\pm0.8$&$8.1\pm0.7$&$7.7\pm0.7$&$\mathbf{8.9\pm0.4 }$&$8.8\pm0.8 $\\
caveflyer&$5.4\pm0.8$&$6.3\pm0.6 $&$6.0\pm0.6$&$4.6\pm0.9$&$6.3\pm0.5 $&$\mathbf{6.8\pm0.7 }$\\
chaser&$5.2\pm0.7$&$4.9\pm1.0$&$5.7\pm1.1$&$6.8\pm0.9 $&$6.9\pm1.2 $&$\mathbf{8.0\pm0.6 }$\\
climber&$5.9\pm0.6$&$6.0\pm0.8$&$6.6\pm0.7 $&$6.4\pm0.9$&$6.3\pm0.8$&$\mathbf{6.8\pm0.7 }$\\
coinrun&$8.6\pm0.4$&$\mathbf{9.2\pm0.2 }$&$8.6\pm0.3$&$8.6\pm0.4$&$8.8\pm0.5$&$9.0\pm0.4$\\
dodgeball&$1.7\pm0.2$&$1.2\pm0.4 $&$1.8\pm0.4$&$5.1\pm1.6 $&$1.8\pm0.5$&$\mathbf{10.3\pm1.4 }$\\
fruitbot&$27.3\pm0.9$&$27.1\pm1.6$&$27.7\pm0.8$&$27.0\pm1.3$&$28.0\pm1.3$&$27.6\pm1.5$\\
heist&$2.8\pm0.9$&$2.5\pm0.6$&$2.7\pm0.4$&$3.2\pm0.7$&$2.9\pm0.5$&$\mathbf{4.9\pm1.3 }$\\
jumper&$5.7\pm0.4$&$6.1\pm0.6$&$6.1\pm0.3 $&$5.6\pm0.5$&$5.8\pm0.5$&$5.9\pm0.3$\\
leaper&$4.2\pm1.3$&$6.4\pm1.2 $&$5.2\pm1.1$&$4.4\pm1.4$&$6.8\pm1.2 $&$\mathbf{8.7\pm1.0 }$\\
maze&$5.5\pm0.4$&$5.0\pm0.3 $&$5.4\pm0.5$&$6.2\pm0.5 $&$5.5\pm0.8$&$\mathbf{7.2\pm0.8 }$\\
miner&$8.7\pm0.7$&$8.9\pm0.6$&$9.5\pm0.4 $&$\mathbf{10.1\pm0.6 }$&$9.6\pm0.6 $&$10.0\pm0.5 $\\
ninja&$6.0\pm0.4$&$6.8\pm0.5 $&$6.9\pm0.5 $&$5.8\pm0.8$&$\mathbf{7.2\pm0.4 }$&$7.0\pm0.5 $\\
plunder&$5.1\pm0.6$&$5.9\pm1.1$&$5.7\pm0.5 $&$7.8\pm0.9 $&$\mathbf{8.7\pm2.2 }$&$7.7\pm0.9 $\\
starpilot&$26.8\pm1.5$&$19.8\pm3.4 $&$\mathbf{32.7\pm1.5 }$&$31.7\pm2.4 $&$27.9\pm4.4$&$29.6\pm2.2 $\\
\midrule
Normalized test returns (\%)&$100.0\pm4.5$&$103.0\pm3.6$&$113.8\pm2.8 $&$129.8\pm8.2 $&$128.3\pm5.8 $&$\mathbf{176.4\pm6.1 }$\\
\midrule
\addlinespace[0.25cm]
MultiRoom-N4-Random & $0.80\pm0.04$ & -- & -- & -- & $\mathbf{0.81\pm0.01}$ & -- \\
ObstructedMazeGamut-Easy&$0.53\pm0.04$& -- & -- & -- & $\mathbf{0.85\pm0.04}$& -- \\
ObstructedMazeGamut-Med&$0.65\pm0.01$& -- & -- & -- & $\mathbf{0.73\pm0.07}$& -- \\
\midrule
Normalized test returns (\%)&$100.0\pm2.5$& -- & -- & -- &$\mathbf{124.3\pm4.7}$ & --\\
\bottomrule
\end{tabular}
\end{subtable}
\end{center}
\end{table*}

\subsection{MiniGrid}
\label{subsection:minigrid_results}
\begin{figure*}
    \centering
    \begin{subfigure}[b]{.9\textwidth}
        \includegraphics[width=\textwidth]{figures/plots/minigrid-test-returns-v4.pdf}
        \label{fig:multiroom-value-testreturns}
    \end{subfigure}\vspace{-1em}
    \begin{subfigure}[b]{0.9\textwidth}
        \includegraphics[width=\textwidth]{figures/plots/minigrid-curricula.pdf}
        \label{fig:minigrid-autocurricula-final}
    \end{subfigure}
    \vspace{-.5cm}
    \caption{Top: Mean episodic test returns of \algoabbrev{} and the uniform-sampling baseline on MultiRoom-N4-Random (4 runs), ObstructedMazeGamut-Easy (3 runs), and ObstructedMazeGamut-Medium (3 runs). Bottom: The probability mass assigned to levels of varying difficulty over the course of training for the respective environment for a single run.
    }
    \label{fig:minigrid-results}
\end{figure*}

We provide empirical support for the Value Correction Hypothesis (defined in Section \ref{methods:plr}) on hard exploration environments in MiniGrid, whose levels clearly separate into discrete, qualitatively different difficulties. As in the case of Procgen Benchmark, \algoabbrev{} with rank prioritization significantly improves sample efficiency and generalization. Further, these improvements demonstrate our method's applicability to discrete state spaces. On these MiniGrid environments, we find a slightly higher staleness coefficient of $\rho = 0.3$ leads to better test performance. The results are summarized in the top row of Figure~\ref{fig:minigrid-results}.

For evaluation purposes, we bin each level into its corresponding difficulty, expressed as ascending, discrete values (note that \algoabbrev{} does not have access to this privileged information). From Figure~\ref{fig:minigrid-results} we see how the expected difficulty of levels sampled using \algoabbrev{} changes throughout training for each environment. We observe that as level weights are updated based on the agent's past experiences of each level, these levels become sampled according to an implicit curriculum over the training levels that prioritizes progressively harder levels. 
Notably, \algoabbrev{} struggles to discover a useful curriculum for around the first $4{,}000$ updates on ObstructedMazeGamut-Medium, at which point it discovers a curriculum that gradually assigns more weight to harder levels. This curriculum enables \algoabbrev{} with access to only $6{,}000$ training levels to attain even higher mean test returns than the uniform-sampling baseline with access to the full set of training levels, of which there are roughly $4$ billion by our estimate (so our training levels constitute $0.00015\%$ of the total number).


==> core/archive/results_table_old.tex <==
\begin{subtable}{\linewidth}
\centering
\begin{tabular}{l|r r r| r r}
\toprule
Environment &Uniform &TSCL &UCB-DrAC &PLR &UCB-DrAC + PLR\\
\midrule
BigFish&$3.72\pm1.24$&$4.34\pm1.32$&$8.73\pm1.13$&$10.91\pm2.81$&$\mathbf{14.28\pm2.12}$\\
BossFight&$7.7\pm0.37$&$7.42\pm0.75$&$7.65\pm0.67$&$\mathbf{8.94\pm0.35}$&$8.84\pm0.8$\\
CaveFlyer&$5.37\pm0.79$&$6.26\pm0.62$&$4.61\pm0.93$&$6.32\pm0.47$&$\mathbf{6.76\pm0.7}$\\
Chaser&$5.23\pm0.69$&$4.95\pm0.97$&$6.79\pm0.93$&$6.9\pm1.21$&$\mathbf{8.01\pm0.6}$\\
Climber&$5.93\pm0.6$&$5.99\pm0.79$&$6.39\pm0.92$&$6.33\pm0.84$&$\mathbf{6.8\pm0.67}$\\
CoinRun&$8.62\pm0.4$&$\mathbf{9.2\pm0.18}$&$8.62\pm0.45$&$8.76\pm0.47$&$8.95\pm0.37$\\
Dodgeball&$1.69\pm0.23$&$1.22\pm0.38$&$5.11\pm1.65$&$1.78\pm0.46$&$\mathbf{10.33\pm1.36}$\\
% FruitBot&$27.29\pm0.94$&$27.1\pm1.65$&$27.02\pm1.35$&$\mathbf{28.02\pm1.35}$&$27.62\pm1.47$\\
FruitBot&$27.29\pm0.94$&$27.1\pm1.65$&$27.02\pm1.35$&$28.02\pm1.35$&$27.62\pm1.47$\\
Heist&$2.77\pm0.92$&$2.46\pm0.56$&$3.17\pm0.74$&$2.93\pm0.48$&$\mathbf{4.93\pm1.3}$\\
% Jumper&$5.71\pm0.42$&$\mathbf{6.12\pm0.6}$&$5.61\pm0.46$&$5.83\pm0.48$&$5.86\pm0.34$\\
Jumper&$5.71\pm0.42$&$6.12\pm0.6$&$5.61\pm0.46$&$5.83\pm0.48$&$5.86\pm0.34$\\
Leaper&$4.18\pm1.33$&$6.37\pm1.22$&$4.44\pm1.42$&$6.83\pm1.15$&$\mathbf{8.66\pm0.98}$\\
Maze&$5.46\pm0.37$&$4.97\pm0.32$&$6.21\pm0.5$&$5.49\pm0.8$&$\mathbf{7.23\pm0.82}$\\
Miner&$8.73\pm0.72$&$8.92\pm0.59$&$\mathbf{10.09\pm0.6}$&$9.56\pm0.62$&$10.03\pm0.54$\\
Ninja&$6.04\pm0.41$&$6.78\pm0.54$&$5.83\pm0.79$&$\mathbf{7.24\pm0.38}$&$6.96\pm0.5$\\
Plunder&$5.05\pm0.55$&$5.9\pm1.14$&$7.79\pm0.89$&$\mathbf{8.68\pm2.18}$&$7.67\pm0.95$\\
StarPilot&$26.84\pm1.54$&$19.81\pm3.41$&$\mathbf{31.68\pm2.36}$&$27.9\pm4.35$&$29.64\pm2.22$\\
\midrule
Normalized test returns (\%)&$100.0\pm4.5$&$103.0\pm3.6$&$129.8\pm8.2$&$128.3\pm5.8$&$\mathbf{176.4\pm6.1}$\\
\midrule
\addlinespace[0.25cm]
MultiRoom-N4-Random & $0.80\pm0.04$ & -- & -- & $\mathbf{0.81\pm0.01}$ & -- \\
ObstructedMazeGamut-Easy&$0.53\pm0.04$& -- & -- & $\mathbf{0.85\pm0.04}$& -- \\
ObstructedMazeGamut-Medium&$0.65\pm0.01$& -- & -- & $\mathbf{0.73\pm0.07}$& -- \\
\midrule
Normalized test returns (\%)&$100.0\pm2.5$& -- & -- &$\mathbf{124.3\pm4.7}$ & --\\
\bottomrule
\end{tabular}
\end{subtable}
